I'm Spartacus, No, I'm Spartacus: Measuring and Understanding LLM Identity Confusion

Large Language Models (LLMs) excel in diverse tasks such as text generation, data analysis, and software development, making them indispensable across domains like education, business, and creative industries. However, the rapid proliferation of LLMs (with over 560 companies developing or deploying them as of 2024) has raised concerns about their originality and trustworthiness. A notable issue, termed identity confusion, has emerged, where LLMs misrepresent their origins or identities. This study systematically examines identity confusion through three research questions: (1) How prevalent is identity confusion among LLMs? (2) Does it arise from model reuse, plagiarism, or hallucination? (3) What are the security and trust-related impacts of identity confusion? To address these, we developed an automated tool combining documentation analysis, self-identity recognition testing, and output similarity comparisons--established methods for LLM fingerprinting--and conducted a structured survey via Credamo to assess its impact on user trust. Our analysis of 27 LLMs revealed that 25.93% exhibit identity confusion. Output similarity analysis confirmed that these issues stem from hallucinations rather than replication or reuse. Survey results further highlighted that identity confusion significantly erodes trust, particularly in critical tasks like education and professional use, with declines exceeding those caused by logical errors or inconsistencies. Users attributed these failures to design flaws, incorrect training data, and perceived plagiarism, underscoring the systemic risks posed by identity confusion to LLM reliability and trustworthiness.

==> sections/sec1-introduction.tex <==
\section{Introduction}

The rapid development of large language models(LLMs) has significantly advanced the state of the art in natural language processing, enabling a wide range of applications from automated translation to conversational AI. However, alongside these advancements, there has been a growing concern regarding the intellectual property rights of these models. One particular issue that has emerged is the potential for plagiarism or unauthorized use, where some models may leverage the APIs or architectures of other models without proper acknowledgment or licensing. For instance, models might directly call the API of another model without disclosing this fact or use pre-trained weights from other models without explicit permission.
The expense associated with training large language models from scratch is considerable. For instance, the training cost of the Llama-2 models, requiring 3,311,616 GPU hours on the NVIDIA A100-80GB GPU\cite{t2}, can reach into the tens of millions of dollars. As a result, numerous companies have opted for the fine-tuning of pre-trained models. Advancements in fine-tuning methodologies, such as Low-Rank Adaptation (LoRA)\cite{t3}, have made it feasible for ordinary users to adapt these models to their specific requirements.As of September 2024, the platform "Hugging Face" hosts over 18,000 models related to LLAMA2, indicating a significant adoption and development within the community. Furthermore, it is noted that some entities may utilize the architectural designs or training datasets of open-source models to construct their own proprietary models without public acknowledgment. Such practices can pose a risk to the original model owners by undermining their contributions and potentially infringing upon their intellectual property rights.

In recent years, alongside the advancement of LLMs, there has been an emergence of unethical phenomena.For instance, the open-source large language model Yi-34B\cite{t1}, developed by 01.AI, was noted to have utilized the architecture of Meta's open-source model LLaMA\cite{t2} entirely, with modifications limited to the names of only two tensors. Similarly, Llama3-V, an open-source model released by an AI team composed of students from Stanford University in the United States, was found to share virtually identical model architecture and code with MiniCPM-Llama3-V 2.5, an open-source achievement by the Chinese large model company MianBi Intelligence. These findings have sparked allegations of "plagiarism".

% In traditional machine learning models, copyright protection is typically addressed through two main approaches: watermarking and fingerprinting. Watermarking involves embedding signatures into the model either by inserting backdoors into the training dataset or modifying the model itself. This approach requires altering the model, which can be intrusive, and it is primarily a preventive measure that is not applicable to models that have already been released publicly. On the other hand, fingerprinting protects models in a non-intrusive manner by extracting unique properties of the model and verifying them against a database of registered fingerprints.

For attacker models, white-box detection schemes require knowledge of the model's internal details, such as parameters and architecture, which can be challenging to obtain for LLMs due to their massive structures. In contrast, black-box protection schemes are more practical for users since they do not require deploying the entire model on the user's side, which can be cost-prohibitive. Existing detection methods for victim models are based on white-box implementations.

In this work, we introduce XX, a fully black-box copyright protection scheme for large language models based on fingerprinting. Our proposed method offers several key advantages:

Non-intrusiveness: It does not interfere with the original training process of the model.
Flexibility: It does not require any information about the model architecture or parameters of either the victim or attacker models, making it suitable for black-box scenarios.

The main contributions of this paper are summarized as follows: 
\begin{itemize}
\item We propose XX, an entirely automated pipeline designed for the detection of similarities among various LLMs. This system is engineered to analyze potential instances of plagiarism and other unethical phenomena within the domain of artificial intelligence linguistics. 

\item We integrate LLMs into our automated process, leveraging their capabilities to assist in the extraction and analysis phases. 

\item Our methodology is entirely black-box in nature, requiring no information regarding the weights or architectures of either the victim or the attacker models. This approach ensures that our analysis and detection mechanisms are independent of the internal structures and parameters of the models under investigation, thereby enhancing the versatility and applicability of our system across diverse model types and frameworks.

\item Our experimental results indicate instances of suspected plagiarism in certain models. We analyze these findings and discuss possible alternative explanations.
\end{itemize}
The remainder of this paper is organized as follows: Section 2 provides a detailed overview of Background. Section 3 describes our proposed method, including the technical details and implementation. Section 4 presents experimental results demonstrating the effectiveness of our approach. Finally, Section 5 concludes the paper and outlines directions for future research.

==> sections/sec7-relatedwork.tex <==
\subsection{Related Works}
Direct Parameter Comparison:
Direct parameter comparison is a straightforward method for assessing the similarity between two machine learning models. This approach involves comparing the values of the model's parameters directly. If the parameters of two models are identical or nearly identical, it suggests that the models are the same or very similar. However, this method can be easily evaded by retraining a model with slight variations, which can change the parameter values while maintaining the model's functionality.

Intrusive Watermarking Techniques:
Intrusive watermarking techniques involve modifying the original model in a way that embeds a unique signature or watermark. This modification can affect the model's parameters, architecture, or both. The watermark is designed to be robust against various attacks and modifications, making it difficult to remove without altering the model's performance. The embedding process can sometimes impact the model's accuracy, especially if the watermark is too strong or if the model is small.

Non-Intrusive Fingerprinting Techniques:
Non-intrusive fingerprinting techniques do not modify the original model but rather extract a set of unique attributes or characteristics that serve as a "fingerprint" of the model. These attributes can be derived from the model's behavior, such as its outputs on specific inputs, or from other mechanisms that capture the model's unique properties. The fingerprinting process is designed to be non-intrusive, meaning it does not alter the model's functionality or performance. During the verification phase, the fingerprint is compared with that of a suspect model to determine if they are similar, indicating potential derivation or copying.
